A Survey on Error-Bounded Lossy Compression for Scientific Datasets

Error-bounded lossy compression has been effective in significantly reducing the data storage/transfer burden while preserving the reconstructed data fidelity very well. Many error-bounded lossy compressors have been developed for a wide range of parallel and distributed use cases for years. They are designed with distinct compression models and principles, such that each of them features particular pros and cons. In this paper we provide a comprehensive survey of emerging error-bounded lossy compression techniques. The key contribution is fourfold. (1) We summarize a novel taxonomy of lossy compression into 6 classic models. (2) We provide a comprehensive survey of 10 commonly used compression components/modules. (3) We summarized pros and cons of 46 state-of-the-art lossy compressors and present how state-of-the-art compressors are designed based on different compression techniques. (4) We discuss how customized compressors are designed for specific scientific applications and use-cases. We believe this survey is useful to multiple communities including scientific applications, high-performance computing, lossy compression, and big data.

==> tex/05_compression_accelerator.tex <==
\section{Lossy Compression for Accelerator Devices}
\label{sec:compression_accelerator}

\subsection{GPU-Supported Lossy Compression}
%Boyuan Zhang, Jiannan Tian, and Yafan Huang

\begin{table}[h]
    \centering
    \footnotesize
    \caption{GPU-Supported Error-Bounded Compressors and Corresponding Compression Pipelines}  \vspace{-2mm}  
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    Compressor&BirthYear&Compression Pipeline&Domain&References\\
    \hline
    cuZFP& & PDT+OWT+BPC & & \cite{cuZFP}\\ \hline
    cuSZ& & QT+PDP+HE+RE& & \cite{cusz,cuszplus}\\ \hline
    cuSZx& & & & \cite{szx}\\
    \hline
    GPU-MGARD& 2021 & PDP+QT+HE+RE & Generic & \cite{chen2021accelerating, gong2023mgard} \\ \hline
    FZ-GPU& & & & \cite{zhang2023fz}\\ \hline    
    cuSZp& 2023 & CE+QT+PDP+FE & Generic & \cite{huang2023cuszp}\\ \hline    
    cuSZ-I & 2023 & PDP+QT+HE+NB&Generic & \\ \hline
    \end{tabular}
    \label{tab:gpu-pipelines}
\end{table}
\subsubsection{cuZFP}
%Dingwen Tao

\subsubsection{\scshape cuSZ}

%% jtian: the text is modified from the previous survey.
{\scshape cuSZ}~~\cite{cusz,cuszplus} is the first error-bounded lossy compressor on GPUs, adapting the SZ framework for scientific data. {\scshape cuSZ} provides a practical framework on GPUs. The practicality lies in the balanced design aiming at achieving high throughput while maintaining good data rate distortion (compression-ratio-to-quality) correspondence. This GPU-based framework is also the basis of  subsequent work: FZ-GPU, cuSZp, and {\scshape cuSZ-I}.

The basic framework contains the fully parallelized Lorenzo-based prediction-quantization and coarse-grained multibyte symbol-enumerating Huffman encoding, with a further lossless encoding. The lossless encoding can be dropped for  subsequent high throughput. 
The key novelty of {\scshape cuSZ}, on top of the practice on GPUs, is the demonstration that the achieved capability originates from both the algorithm design and the performance optimization in a hardware-software co-design manner, which are detailed in {\scshape cuSZ} work~\cite{cusz,cuszplus}. In addition, the accelerated Huffman encoding~\cite{revisiting-huffman}, which has yet to be integrated into {\scshape cuSZ}, can be a powerful way to improve the end-to-end throughput because of its fast encoding capability.

\subsubsection{cuSZx}
%Xiaodong Yu
cuSZx~\cite{szx} is a highly optimized GPU-based implementation of SZx design. It assigns different data blocks in SZx to different CUDA thread blocks and uses different CUDA threads to process different data points in a data block, in order to avoid expensive grid-level synchronization and communication. %During the compression, the CUDA warp-level operations are leveraged to compute the $\mu$ and radius of the assigned data block. For a constant block, the thread block will record the $\mu$ and immediately move forward. The nonconstant block will be further processed in the one CUDA thread compressing one data point style. During the decompression, only the nonconstant blocks are heavy enough to be decompressed in the GPU. Since decompression is the reverse of compression, its implementation is mostly similar to the above design. 
Some generic GPU optimization techniques have been applied to improve the overall performance, including using CUDA vector types (e.g., char4) to maximize the memory bandwidth usage and leveraging shared memory to optimal bytewise manipulation of floating-point values and to work around the missing of \textit{union} data structure on the GPU.
%GAIL - do you mean union-find

Two types of dependencies, address dependency and data value dependency,  exist during compressing and decompressing nonconstant blocks. Two solutions are provided in cuSZx to break these dependencies. First, it adds an additional prefix-scan step to the compressor and decompressor, so that the address dependency is eliminated and all threads can sync and communicate to find their own starting address. Prefix-scan can be efficiently parallelized on GPUs by using two-level in-warp shuffles~\cite{scan}. Second, it proposes a novel \emph{index-propagation} approach to identify the dependency chains in the parallel fashion. Dependency chains can help break the data value dependencies by guiding the leading byte retrieval. This approach is inexpensive since it uses only  lightweight shuffle operations with the recursive doubling style. 

\subsubsection{GPU-MGARD}
%Xin Liang
GPU-MGARD~\cite{chen2021accelerating, gong2023mgard} is a performant, portable, and extendable implementation of the MGARD algorithms on GPUs. 
It follows the same compression algorithm as MGARD with highly optimized GPU kernels.
Specifically, it includes (1) a grid-processing kernel for efficient manipulation of the operations in the hierarchical grids, which reduces the thread divergences through decoupling memory access with thread-node assignment for computation;
(2) a linear-processing kernel that accelerates the decomposition algorithm through out-of-place computation, operation merges, cache with shared memory, and kernel fusion; and (3) an iterative-processing kernel that ensures coalesced memory access patterns with concurrent memory accesses via a dynamic data-thread assignment strategy. 
In addition, GPU-MGARD provides heuristics to autotune the execution parameter based on a theoretical performance model built for the algorithm, which further improves the end-to-end performance. 
Other features of GPU-MGARD include unified APIs for compression and refactoring operations on different CPU/GPU architectures, self-describing data format, and multidevice out-of-core processing. 

\subsubsection{FZ-GPU}
%Boyuan Zhang

FZ-GPU\cite{zhang2023fz} is designed as a high-performance, lossy compression tool for scientific datasets on GPU platforms. The architecture confronts a common throughput limitation found in SZ-based GPU compressors, which stems from the integration of Huffman encoding---a process not optimally aligned with GPU's computational strengths because of its inherently slow execution. To solve this inefficiency, FZ-GPU introduces a fast compression pipeline. This approach replaces the traditional, sluggish Huffman encoding with a combination of bitshuffle operations and swift lossless encoding mechanisms, thereby enhancing performance.

In a more detailed examination, FZ-GPU employs the cuSZ's advanced prediction-quantization kernel for executing Lorenzo prediction and quantization on input floating-point data. This process transforms the original floating-point values into integer forms, effectively mitigating spatial data redundancy. Notably, FZ-GPU introduces a modification in the representation of quantization codes: the initial bit signifies the sign, while the remaining bits are unchanged. This alteration aims to address the reduction of bit-level sparsity encountered with negative values and those proximate to zero, a scenario exacerbated by the conventional use of 2's complement. Subsequently, FZ-GPU utilizes a specialized GPU bitshuffle kernel designed to reorder data bits, targeting integers near zero to further diminish bit-level sparsity. This step is complemented by warp-level optimizations to bolster the performance of bit-level operations. Culminating the process, FZ-GPU integrates a fast, embarrassingly parallel lossless encoding technique to realize significant throughput gains.

This comprehensive redesign of the compression pipeline by FZ-GPU not only addresses the inefficiencies associated with Huffman encoding on GPUs but also establishes a more effective method for managing scientific data compression, leveraging the inherent strengths of GPU architectures for enhanced performance. However, the compression ratio is, on average, marginally lower when compared with cuSZ.

\subsubsection{cuSZp}
cuSZp~\cite{huang2023cuszp} is another prediction-based error-bounded lossy compression with fused kernel. It performs compression/decompression in a single GPU function without any CPU computations, achieving ultrafast end-to-end throughput.
Given an original HPC dataset, cuSZp splits it into a set of 1D data blocks (e.g., 32 consecutive floating-point values) and performs the compression pipeline in four major steps: (1) zero-block recognition (CE) uses only one byte to represent a data block with all zero values; (2) prequantization (QT) transforms each floating-point value into an integer considering the error bounds, and this is also the only lossy step in cuSZp;
(3) lightweight prediction (PDP) then encodes the generated integers in one block with 1D Lorenzo prediction to reduce the number of effective bits;
and (4) fixed-length encoding (FE) is adopted to pack effective bits densely within each data block.
Besides these  steps, cuSZp  decodes the linear recurrence (i.e., prefix-sum problem) across data blocks by a single-pass chained scan and simplifies the program control flow by a blockwise bitshuffle, for optimizing the throughput.
However, cuSZp has a limitation---it processes an HPC dataset with only 1D operations, ignoring high-dimensional spatial localities and cross-block data patterns, leading to limited compression ratio and data qualities, compared with CPU-based lossy compression methods.
\subsubsection{cuSZ-I}
The interpolation-based cuSZ-I [] 
%GAIL - possiblereference is Jinyang Liu, Jiannan Tian, Shixuan Wu, Sheng Di, Boyuan Zhang, Yafan Huang, Kai Zhao, Guanpeng Li, Dingwen Tao,Zizhong Chen, and Granck Cappello, xuSZ-I: High-fidelity Error-Bounded Lossy Copression for Scientific Dat on GPUs, arXivL2312.05492, Dec. 2023
can be regarded as a variant of QoZ [] 
%GAIL - ref 121?
on GPU platforms; and to our best knowledge, it is the first high-ratio scientific error-bounded lossy compression on GPUs while preserving decent compression throughputs. In order to optimize the parallelization on GPUs, several essential customizations have been made on cuSZ-I compared with the CPU-based QoZ. First, it partitions the input data into small data chunks to promote both  inner-threadblock and inter-threadblock parallelization. Second, cuSZ-I integrates a lightweight interpolation autotuning kernel based on both empirical findings and real-time tests for best throughput performance. Third, cuSZ-I uses the fast NVIDIA Bitcomp lossless data encoder [] 
%GAIL - possible ref https://developer.nvidia.com/nvcomp
to substitute the low-throughput Zstd (on GPU platforms). In evaluations, cuSZ-I significantly outperforms any other existing GPU-based scientific lossy compressors in terms of compression rate distortion. For example, it can achieve up to 500\% compression ratio improvement over the second best compressor under the same decompression PSNR. 
\subsection{FPGA-Supported Lossy Compression}
%Kaz, Jiannan Tian, and Dingwen

\subsubsection{GhostSZ}

GhostSZ~\cite{xiong2019ghostsz} is a framework that enhances the SZ lossy compression algorithm by integrating FPGAs. This integration aims to address the challenges of managing large data volumes in HPC environments. By leveraging FPGAs, GhostSZ significantly speeds up the SZ compression process, offering an efficient solution for reducing network traffic and storage requirements in HPC systems. This enhancement is crucial for maintaining high throughput and efficient data handling in these computationally intensive applications.

\subsubsection{WaveSZ}


\subsubsection{ZFP-V}


\subsubsection{DE-ZFP}

%\subsection{Vector-supported Lossy Compression}
%Jon Calhoun

==> tex/07_evaluation.tex <==
%GAIL - Sorry -  I just realized you had commented out in main.tex this section and the next.

\section{Assessment Methodology of Lossy Compression Performance and Quality}
\label{sec:evaluation}
%Mention sdrbench

\subsection{Evaluation Metrics}
Several important quantitative metrics are widely used in the community of scientific lossy compression. They measure and evaluate the scientific lossy compressors in various aspects, including compressed data size, decompressed data quality, and computing efficiency. Here we briefly describe the most representative evaluation metrics.
\begin{itemize}

    \item \textbf{Compression ratio (CR)}: Compression ratio is the metric mostly cared about by  users because it directly measures the size of compressed data. Given the input data denoted as $X$, compressed data denoted as $Z$, and $|\ |$ denoted as the size operator (in bytes), the compression ratio $CR$ is $CR=\frac{|X|}{|Z|}$.
    \item \textbf{Bit rate (BR)}: Bit rate also represents the compressed data size; it is the number of bits in the compressed data for each element in the input data. If we denote the bit rate as $b$, then $b=\frac{8*|Z|}{(|X|/sizeof(x))}=\frac{8*sizeof(x)}{CR}$ ($sizeof(x)$ is the size in bytes of each element $x$ in $X$).
    \item \textbf{Peak signal-to-noise ratio (PSNR)}: PSNR is often used to measure the distortion between the original input data and the decompressed data. It is computed by the input value range and the mean square error between the input data and the decompressed data. If we denote input as $X$ and the decompressed data as $X'$, \cite{z-checker} presents the formula of PSNR as follows:
    \def\formulaPSNR{
    P\hspace{-0.3mm}S\hspace{-0.3mm}N\hspace{-0.3mm}R = 20\log_{10}{vrange(X)} \hspace{-0.3mm}-\hspace{-0.3mm} 10\hspace{-0.3mm}\log_{10}{MSE(X,\hspace{-0.3mm}X')} \hspace{2mm} (vrange=\max(X)-\min(X))
    }
    \vspace{-2mm}
    \begin{equation}
    \label{eq:psnr}
      \formulaPSNR
      \vspace{-1mm}
    \end{equation}
    \noindent
    \item \textbf{Structural similarity index measure (SSIM)}:  SSIM \cite{ssim} is another important metric for assessing the quality of decompressed data, which measures the similarity between the visual quality of input and decompressed data. The formula for calculating SSIM with input data $X$ and decompressed data $X^{'}$ is \cite{ssim}
    \begin{equation}
    \label{eq:ssim}
    \begin{array}{l}
     SSIM = \frac{1}{N}\sum\nolimits_{i = 1}^N {SSIM_i (X,X')}. 
     \end{array}
    \end{equation}
    $SSIM_i(X,X')$ is the calculation of SSIM for a local sliding window $i$ as
    \begin{equation}
    \label{eq:ssim2}
    \begin{array}{l}
    SSIM_i(X,X')=\frac{(2\mu_X\mu_{X'}+c_1)(2\sigma_{XX'}+c_2)}{(\mu_X^2+\mu_{X'}^2+c_1)(\sigma_X^2+\sigma_{X'}^2+c_2)},
     \end{array}
    \end{equation}
    where $\mu$ is the mean and $\sigma$ is the standard variance/covariance. 
    
    \item{\textbf{Autocorrelation of compression error (AC)}}:
    Autocorrelation of compression error  measures the relevance of pointwise decompression errors. In many cases we will want nonrelevant random errors to avoid artifacts and biases brought by errors. The calculation of AC is
    \begin{equation}
    \label{eq:ac}
    \begin{array}{l}
    AC = \frac{{E(e_i  - \mu _i )(e_{i + k}  - \mu _{i + k} )}}{{\sigma ^2 }},
     \end{array}
    \end{equation}
    where $e_i$ denotes the compression error at data point $i$ and $k$ is the lag (or offset) used to calculate the autocorrelation. 

    \item {\textbf{Visualizations}}: Instead of mathematically calculating quality metrics, we usually can directly visualize the input and decompressed data in colored or gray-scale images. With this technique, we can intuitively verify whether the decompressed data meet the requirements of quality.

    \item {\textbf{Compression/decompression speed/time cost}}: Regarding the efficiency of the scientific compression in HPC systems, besides the compression ratio and quality, we should also check the compression/decompression speeds and time costs of compressors.
\end{itemize}

\subsection{Evaluation Methodologies}

According to the aforementioned evaluations for scientific lossy compressions, several different experiments and results can be conducted and presented for the examination, verification, and comparison of the performance and quality of the compressors. In the following, we describe the most representative and widely used evaluation methodologies.

\begin{itemize}
    \item {\textbf{Compression ratio under the same error bound}}: By listing and comparing the compression ratios of different compressors under the same error bound configuration, we can know and rank the capabilities of compressors for reducing the data size. 
    \item {\textbf{Rate-distortion plots}}: Plotting the crucial bit rate and distortion metric (PSNR, SSIM, AC, etc.) curves for compressors can inform us of how well the compressors perform under a certain quality constraint.
    \item {\textbf{Decompression visualization under the same CR}}: Comparing the visualizations of the decompression results from different compressors based on the same CR can verify the preservation of visual quality by each compressor.
    \item {\textbf{Sequential speed profiling}}: To determine the computational cost of each scientific lossy compressor, we need to generate, collect, and organize the data for the sequential execution speeds (both compression and decompression) from each compressor.
    \item {\textbf{Parallel performance profiling}}: Besides the sequential tests, the performance of scientific lossy compressors should also be evaluated in parallel test cases to check their scalability and the estimation of performances on real-world parallel computing tasks.

\end{itemize}
%\subsection{Benchmark datasets}
%who
%\subsection{Toolkits}
%Libpressio?
%\subsection{Evaluations}
%JZZ Todo 
%Platform:  Anvil
%Metric: compression ratio (under fixed eb), bitrate-psnr/ssim, sequential comp/decomp speed
%Compressors: fpzip bitgrooming sz2.1 sz1.4 digitrounding szx (mgard? ask xin).
%Another 7 compressors: HPEZ QoZ1.1 SZ3 ZFP SPERR FAZ TTHRESH
%Datasets: Jinyang will prepare for it 
%config: (VR-REL) ebs (see Jinyang's test repo)
%plots: PSNR-bitrate, SSIM-bitrate, com throughput, decom throughput

%Jinyang's test repo: https://github.com/Meso272/Test_scripts/blob/master/test_sz2.py
%MGARDx: https://github.com/lxAltria/MGARDx
%Anvil tutorial: www.rcac.purdue.edu/knowledge/anvil/run
%example: sinteractive -N1 -n128 -A cis220161

==> tex/08_estimation.tex <==
\section{Estimation of Compression Ratio and Quality}
\label{sec:benchmark}

%Hasan, Sian Jin, Robert?, etc.
% \cite{zemliachenko2015compression, lu2018understanding, di2018efficient,underwood2020fraz,wang2019compression, jin2022improving, ganguli2023lightweight, underwood2023black, wang2023zperf, rahman2023feature, tao2019optimizing, qin2020estimate}
As discussed earlier, existing error-bounded lossy compressors~\cite{tao2017significantly,zhao2021optimizing,zfp,liang2021mgard+} are  designed mainly based on error control mode. Therefore, compression ratio offered by a particular lossy compressor would be known only after the completion of execution of the corresponding lossy compressor based on a scientific dataset. On the one hand, HPC applications/simulations are producing vast volumes of scientific data~\cite{gleckler2016industrial, almgren2013nyx, habib2013hacc}, so compressed data size based on these raw simulation data would still be non-negligible. On the other hand, often scientific users are equipped with limited memory capacity for computation, storage space for storing, and I/O bandwidth for transferring the data. For example, a Summit supercomputer user is usually allocated a limited storage space of 50 TB~\cite{olcf-storage}. Given the juxtaposition of the above two scenarios, it becomes imperative to forecast the compression ratio before the execution of a particular lossy compressor of interest so that allocated resources can be orchestrated more proactively. For example, a crash during compressor execution could be plausible because of the processing of the huge volume of scientific data on the limited memory capacity.

In order to solve the above issue, several recent studies~\cite{lu2018understanding,qin2020estimate,jin2022improving,underwood2023black,ganguli2023lightweight,rahman2023feature} have investigated the interplay of compressor design and data features to accurately and efficiently estimate the compression ratio and quality. While some studies~\cite{lu2018understanding,qin2020estimate} exclusively concentrate on estimating compressibility, others emphasize the assessment of both compressibility and compression quality. For example, Lu et al.~\cite{lu2018understanding} presented a comprehensive  analysis of lossy compression techniques for scientific data. The primary goal was to estimate the compressibility by understanding the intricate relationship between compressor design, data characteristics, and compression effectiveness. The study reveals that factors such as byte entropy, the count of unique bytes, and data correlation significantly impact compressibility. Higher entropy and a greater number of unique bytes result in lower compression ratios, while increased correlation leads to higher compression ratios. The research also indicates that, for compressors with bounded locality like ZFP, accurate and unbiased estimation is achieved through sampling. In contrast, global schemes like SZ require advanced modeling of data features, such as Gaussian model of the distribution of quantization factors, in addition to sampling. This model significantly reduces estimation errors compared with naive sampling. Experiment results show that the estimation accuracy can be up to 99\% for ZFP. On the other hand, for SZ, the average estimation error based on Gaussian model is 29\%. While this approach exhibits commendable accuracy, it entails considerable sampling overhead per dataset. To mitigate this, Qin et al.~\cite{qin2020estimate} proposed a method leveraging deep neural networks to estimate the compressibility of scientific data. This paper is the first study of its kind in that it leverages deep learning for compressibility estimation. Unlike the study proposed by Lu et al.~\cite{lu2018understanding}, this study provides faster performance: the s key design involves extracting both data and compressor-specific features and feeding only these small amounts of features to neural networks for estimation. 
With this method, testing accuracy reaches 94.83\% and 87.47\% for ZFP and SZ, respectively. Incorporating compressor-related features further improves accuracy to 98.86\% for ZFP and 97.01\% for SZ. 

Unlike these studies, which are mainly developed based on  compressor-specific designs, a few other new studies explore the compressibility estimation in a compressor-agnostic manner. For example, Underwood et al.~\cite{underwood2023black} introduced an efficient black-box statistical prediction method for accurately estimating compression ratios based on 2D and 3D scientific datasets. The method involves performing compressor-agnostic statistical analysis on datasets and training a statistical prediction model using measured compression ratios from existing compressors. A key aspect of the proposed method is the formulation of a generic statistical prediction model that does not rely on knowledge of a specific compressor's design principles. The technical contributions include deriving data-based statistical predictors using singular value decomposition, data entropy, and lossless properties via the quantized entropy. The method achieves a median prediction error below 12\%, significantly outperforming other methods while providing a minimum 8.8$\times$ speedup in the search for estimating a specific compression ratio. Ganguli et al.~\cite{ganguli2023lightweight} proposed a statistical features-based method for estimating the compression ratio. They proposed a set of statistical predictors that capture different notions of spatial correlation and smoothness in the dataset, including spatial diversity, spatial correlation, generalized distortion, coding gain, and spatial smoothness. They combined these predictors in a mixture regression model to estimate the compression ratio. The mixture model accounts for heterogeneity and grouping effects in how the predictors relate to compression ratio. It is also the first work to provide statistical bounds on the compression ratio estimates using conformal prediction. The predictors and model fitting are implemented efficiently on GPUs to make the approach lightweight. The overall average median absolute percentage error is 1.2\%. As for efficiency, Ganguli et al. achieves a roughly 3$\times$ performance improvement relative to not using estimates and improvement over the next best method~\cite{underwood2023black}.

On the other hand, it is also important to maintain high data fidelity while achieving high compression ratio for scientific data. Considering both cases, Jin et al.~\cite{jin2022improving} proposed a novel analytical model based on SZ3~\cite{zhao2021optimizing} design principles to efficiently and accurately estimate the compression ratio and data distortion quality for any given dataset. The model aims to avoid the trial-and-error overhead of configuring the lossy compressors. The compression-ratio estimation involves three modules: predictor, quantization, and encoder. The predictor models prediction errors using a designed sampling strategy. The quantization stage estimates error distribution and quantization-code histogram. Compression ratio is then estimated based on theoretical analysis of Huffman encoding and optional lossless compression. For post hoc analysis quality, Jin et al. determined error distribution from the compressor's quantization step and assessed the impact on distortion quality through theoretical derivation of error propagation using hypothetical error injection. The evaluation on 10 scientific datasets shows high accuracy (average 93.47\%) and low computational cost (up to 18.7$\times$ less than trial-and-error-based approach) in estimating the compression ratio and quality.

Additionally, in scientific data management systems, fixed-ratio compression is crucial. The reason is that the systems or management tools frequently require effective data compression while maintaining control over the data size. To achieve this, Rahman et al.~\cite{rahman2023feature} proposed FXRZ, a novel low-cost feature-driven compressor-agnostic framework for fixed-ratio lossy compression of scientific data. Unlike above studies that estimate compressibility, the primary goal of this study was to estimate the error bound based on a target compression ratio. The key design is extracting key data features such as mean value, value range, mean neighbor difference, and mean spline difference to establish a relationship between data characteristics and compressibility. This allows estimating the error bound to reach a target compression ratio without running the compressor, unlike existing trial-and-error approaches. FXRZ incorporates optimizations such as target ratio adjustment and uniform sampling to improve accuracy and performance. Experiments on scientific datasets and state-of-the-art compressors show that FXRZ is highly accurate with only 8.24\% error on average and 108$\times$ faster than prior work. Overall, FXRZ enables efficient fixed-ratio lossy compression by leveraging data features, unlike existing compressor-specific or iterative search techniques.





